The Case for Translation-Invariant Self-Attention in Transformer-Based Language Models

Mechanisms for encoding positional information are central for transformer-based language models. In this paper, we analyze the position embeddings of existing language models, finding strong evidence of translation invariance, both for the embeddings themselves and for their effect on self-attention. The degree of translation invariance increases during training and correlates positively with model performance. Our findings lead us to propose translation-invariant self-attention (TISA), which accounts for the relative position between tokens in an interpretable fashion without needing conventional position embeddings. Our proposal has several theoretical advantages over existing position-representation approaches. Experiments show that it improves on regular ALBERT on GLUE tasks, while only adding orders of magnitude less positional parameters.

==> figures/fig5_large.tex <==
\begin{figure*}[!t]
	\centering
	\hfill
	\begin{subfigure}[t]{0.485\textwidth}
		\centering
		\includegraphics[width=\textwidth, height=5.8cm]{images/test_large-crop.pdf}
		%\caption{$S=5$}
		%\label{sfig:s5}
	\end{subfigure}
	\hfill
	\hfill
	\begin{subfigure}[t]{0.485\textwidth}
		\centering
		\includegraphics[width=\textwidth, height=5.8cm]{images/score_funcs_large-crop.pdf}
		%\caption{$S=1$}
		%\label{sfig:s1}
	\end{subfigure}
	\hfill
	\caption{Positional responses of select attention heads.
	Left: Sections $(\widehat{F}_P)_{i,j}$ through $\widehat{F}_P$ of ALBERT base v2, varying $j$ for 5 different $i$, keeping $j=i$ centered. The sections are similar regardless of $i$ since $\widehat{F}_P$ is close to Toeplitz. Colors distinguish different heads.
	Right: \ours{} scoring functions, attending to similar positions as the heads on the left.
	%Positional responses of all attention heads. Sections through $\widehat{F}_P$ of ALBERT base v2, aligned to the main diagonal, (left) show similar profiles as the corresponding \ours{} scoring functions after finetuning (right).
	Vertical axes differ due to 1) the scaling factor $\sqrt{d_k}$ and 2) softmax being invariant to vertical offset.
	%We first create 5 curves per 4 attention head for of ALBERT base (left) and then show that our model is interpretable by plotting the position scoring functions for 4 attention heads in ALBERT base with \ours{}.
	}
    \label{fig:ffunc_large}
    \vspace{-1em}
\end{figure*}

==> figures/multifix_suppl1.tex <==
\begin{figure*}[h!]
	\centering
	\hfill
	\begin{subfigure}[t]{0.485\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/attention_scores_511.pdf}
		%\caption{$S=1$}
		%\label{sfig:s1}
	\end{subfigure}
	\hfill
	\hfill
	\begin{subfigure}[t]{0.485\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/attention_scores_025.pdf}
		%\caption{$S=5$}
		%\label{sfig:s5}
	\end{subfigure}
	\hfill
	\caption{Plot over the average positional embedding contribution to the attention scores in the attention module for different relative position distances. The plots show that the learned position embeddings in the ALBERT model give rise to sinusoidal contributions to the attention scores, both on macro and micro scales.}
	\label{fig:albert_pos_attention_scores}
    \vspace{-1em}
\end{figure*}

==> figures/multifix_suppl2_albert_regular_att_func.tex <==
\begin{figure*}[b!]
	\centering
	\begin{subfigure}[t]{0.245\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/ALBERT_Attention_Function/attention_weight_functions_00-crop.pdf}
		\caption{Attention head 1}
	\end{subfigure}
	\begin{subfigure}[t]{0.245\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/ALBERT_Attention_Function/attention_weight_functions_01-crop.pdf}
		\caption{Attention head 2}
	\end{subfigure}
	\begin{subfigure}[t]{0.245\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/ALBERT_Attention_Function/attention_weight_functions_02-crop.pdf}
		\caption{Attention head 3}
	\end{subfigure}
	\begin{subfigure}[t]{0.245\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/ALBERT_Attention_Function/attention_weight_functions_03-crop.pdf}
		\caption{Attention head 4}
	\end{subfigure}
	\begin{subfigure}[t]{0.245\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/ALBERT_Attention_Function/attention_weight_functions_04-crop.pdf}
		\caption{Attention head 5}
	\end{subfigure}
	\begin{subfigure}[t]{0.245\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/ALBERT_Attention_Function/attention_weight_functions_06-crop.pdf}
		\caption{Attention head 6}
	\end{subfigure}
	\begin{subfigure}[t]{0.245\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/ALBERT_Attention_Function/attention_weight_functions_08-crop.pdf}
		\caption{Attention head 7}
	\end{subfigure}
	\begin{subfigure}[t]{0.245\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/ALBERT_Attention_Function/attention_weight_functions_07-crop.pdf}
		\caption{Attention head 8}
	\end{subfigure}
	\begin{subfigure}[t]{0.245\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/ALBERT_Attention_Function/attention_weight_functions_08-crop.pdf}
		\caption{Attention head 9}
	\end{subfigure}
	\begin{subfigure}[t]{0.245\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/ALBERT_Attention_Function/attention_weight_functions_09-crop.pdf}
		\caption{Attention head 10}
	\end{subfigure}
	\begin{subfigure}[t]{0.245\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/ALBERT_Attention_Function/attention_weight_functions_10-crop.pdf}
		\caption{Attention head 11}
	\end{subfigure}
	\begin{subfigure}[t]{0.245\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/ALBERT_Attention_Function/attention_weight_functions_11-crop.pdf}
		\caption{Attention head 12}
	\end{subfigure}
	\caption{Rows from the positional attention matrices for all ALBERT base v2 attention heads in the first layer, centered on the main diagonal. Note that the vertical scale generally differs between plots. The plots are essentially sections through the matrices in Fig.\ \ref{fig:allheadmatrices}, but zoomed in to show details of short relative distances, since this is where the main peaks are located, and the highest values are by far the most influential on softmax attention.}
    \vspace{-1em}
\end{figure*}

==> figures/multifix_suppl4_albert_EpEpT.tex <==
\begin{figure*}[ht!]
	\centering
	\begin{subfigure}[t]{0.245\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/EpEpT/albert-base-v1-crop.pdf}
	    \caption{ALBERT base v1}
	\end{subfigure}
	\begin{subfigure}[t]{0.245\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/EpEpT/albert-base-v2-crop.pdf}
	    \caption{ALBERT base v2}
	\end{subfigure}
	\begin{subfigure}[t]{0.245\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/EpEpT/albert-large-v1-crop.pdf}
	    \caption{ALBERT large v1}
	\end{subfigure}
	\begin{subfigure}[t]{0.245\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/EpEpT/albert-large-v2-crop.pdf}
	    \caption{ALBERT large v2}
	\end{subfigure}
	\begin{subfigure}[t]{0.245\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/EpEpT/albert-xlarge-v1-crop.pdf}
	    \caption{ALBERT xlarge v1}
	\end{subfigure}
	\begin{subfigure}[t]{0.245\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/EpEpT/albert-xlarge-v2-crop.pdf}
	    \caption{ALBERT xlarge v2}
	\end{subfigure}
	\begin{subfigure}[t]{0.245\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/EpEpT/albert-xxlarge-v1-crop.pdf}
	    \caption{ALBERT xxlarge v1}
	\end{subfigure}
	\begin{subfigure}[t]{0.245\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/EpEpT/albert-xxlarge-v2-crop.pdf}
	    \caption{ALBERT xxlarge v2}
	\end{subfigure}
	\caption{Visualizations of inner product matrix $P = E_P E_P^T \in \real^{n \times n}$ for $v1$ and $v2$ of different ALBERT models \cite{lan2020albert}. We plot both v1 and v2 to show the progression towards increased Toeplitzness during training.}
    \vspace{-0.5em}
\end{figure*}
